Beyond Rule-based Named Entity Recognition and Relation Extraction for Process Model Generation from Natural Language Text

Process-aware information systems offer extensive advantages to companies, facilitating planning, operations, and optimization of day-to-day business activities. However, the time-consuming but required step of designing formal business process models often hampers the potential of these systems. To overcome this challenge, automated generation of business process models from natural language text has emerged as a promising approach to expedite this step. Generally two crucial subtasks have to be solved: extracting process-relevant information from natural language and creating the actual model. Approaches towards the first subtask are rule based methods, highly optimized for specific domains, but hard to adapt to related applications. To solve this issue, we present an extension to an existing pipeline, to make it entirely data driven. We demonstrate the competitiveness of our improved pipeline, which not only eliminates the substantial overhead associated with feature engineering and rule definition, but also enables adaptation to different datasets, entity and relation types, and new domains. Additionally, the largest available dataset (PET) for the first subtask, contains no information about linguistic references between mentions of entities in the process description. Yet, the resolution of these mentions into a single visual element is essential for high quality process models. We propose an extension to the PET dataset that incorporates information about linguistic references and a corresponding method for resolving them. Finally, we provide a detailed analysis of the inherent challenges in the dataset at hand.

==> 61-bellan-basic-analysis-tables.tex <==


\begin{table}[htb]
\begin{tabularx}{\textwidth}{lYYYYYYY}
\hline                                                                                                      
                                            &                   & \textit{Activity}         &                   & \textit{Further}              & \textit{XOR}          & \textit{AND}          & \textit{Cond.}            \\
                                            & \textit{Activity} & \textit{Data}             & \textit{Actor}    & \textit{Spec.}            & \textit{Gateway}      & \textit{Gateway}      & \textit{Spec.}                \\
\hline
absolute count                              & 501               & 451                       & 439               & 64                            & 117                   & 8                     & 80                            \\
relative count                              & 30.16\%           & 27.21\%                   & 26.43\%           & 3.86\%                        & 7.04\%                & 0.48\%                & 4.82\%                        \\
per document                                & 11.13             & 10.04                     & 9.76              & 1.42                          & 2.60                  & 0.18                  & 1.78                          \\
per sentence                                & 1.20              & 1.08                      & 1.05              & 0.15                          & 0.28                  & 0.02                  & 0.19                          \\
average length                              & 1.10              & 3.49                      & 2.32              & 5.19                          & 1.26                  & 2.12                  & 6.04                          \\
standard dev.                               & 0.48              & 2.47                      & 1.11              & 3.40                          & 0.77                  & 1.54                  & 3.04                          \\
\hline
\end{tabularx}

\caption{
    \label{tab:pet-basic-mention-stats}
    Basic analysis for mentions in the PET dataset done by \cite{bellan2023pet}
}
\end{table}

\begin{table}[htb]
\begin{tabularx}{\textwidth}{lYYYYYY}
\hline
                                            &                   &                       & \textit{Actor}            & \textit{Actor}            & \textit{Further}              & \textit{Same}             \\
                                            & \textit{Flows}    & \textit{Uses}         & \textit{Performer}        & \textit{Recipient}        & \textit{Specific.}            & \textit{Gateway}          \\
\hline
absolute count                              & 674               & 468                   & 312                       & 164                       & 64                            & 42                        \\
relative count                              & 39.10\%           & 27.15\%               & 18.10\%                   & 9.51\%                    & 3.71\%                        & 2.44\%                    \\
per document                                & 15.31             & 10.60                 & 6.96                      & 3.64                      & 1.42                          & 0.96                      \\
per sentence                                & 1.65              & 1.14                  & 0.75                      & 0.39                      & 0.15                          & 0.10                      \\        
\hline
\end{tabularx}


\caption{
    \label{tab:pet-basic-relation-stats}
    Basic analysis for relations in the PET dataset done by \cite{bellan2023pet}
}
\end{table}

==> 62-ablation-study-results.tex <==
\begin{table}[htb]
    \begin{subtable}[t]{.3\linewidth}
        \centering
        \begin{tabular}[t]{lccc}
        
        \hline
        \multicolumn{4}{c}{Scenario \textbf{(1)}}                                           \\
        \hline
                                    & $P$               & $R$               & $F_{1}$       \\
        \hline
        CRF                     & .33               & .33               & .33               \\
        \hline
        
        \end{tabular}
        \caption{Mention extraction in scenario \textbf{(4)}, using raw text as input.}
        \label{tab:pet-module-isolation-mentions}
    \end{subtable}%
    \hfill%
    \begin{subtable}[t]{.3\linewidth}
        \centering
        \begin{tabular}[t]{lccc}
        
        \hline
        \multicolumn{4}{c}{Scenario \textbf{(2)}}                                           \\
        \hline
                                    & $P$               & $R$               & $F_{1}$       \\
        \hline
        Naive                     & .33               & .33               & .33           \\
        Neural                    & .33               & .33               & .33           \\
        \hline
    
        \noalign{\vskip 5mm}   
        
        \hline
        \multicolumn{4}{c}{Scenario \textbf{(3)}}                                           \\
        \hline
                                    & $P$               & $R$               & $F_{1}$       \\
        \hline
        Naive                     & .33               & .33               & .33           \\
        Neural                    & .33               & .33               & .33           \\
        \hline
        
        \end{tabular}
        \caption{Relation extraction in scenarios ground-truth entities \textbf{(4)}, predicted entities, ground-truth mentions \textbf{(5)}, and predicted entities, predicted mentions \textbf{(6)}.}
        \label{tab:pet-module-isolation-entities}
    \end{subtable}%
    \hfill%
    \begin{subtable}[t]{.3\linewidth}
        \centering
        \begin{tabular}[t]{lccc}
        
        \hline
        \multicolumn{4}{c}{Scenario \textbf{(4)}}                                           \\
        \hline
                                    & $P$               & $R$               & $F_{1}$       \\
        \hline
        Rule-Based                     & .33               & .33               & .33           \\
        CatBoost                    & .33               & .33               & .33           \\
        \hline
    
        \noalign{\vskip 5mm}   
        
        \hline
        \multicolumn{4}{c}{Scenario \textbf{(5)}}                                           \\
        \hline
                                    & $P$               & $R$               & $F_{1}$       \\
        \hline
        Rule-Based                     & .33               & .33               & .33           \\
        CatBoost                    & .33               & .33               & .33           \\
        \hline
    
        \noalign{\vskip 5mm}   
        
        \hline
        \multicolumn{4}{c}{Scenario \textbf{(6)}}                                           \\
        \hline
                                    & $P$               & $R$               & $F_{1}$       \\
        \hline
        Rule-Based                     & .33               & .33               & .33           \\
        CatBoost                    & .33               & .33               & .33           \\
        \hline
        
        \end{tabular}
        \caption{Relation extraction in scenarios ground-truth entities \textbf{(4)}, predicted entities, ground-truth mentions \textbf{(5)}, and predicted entities, predicted mentions \textbf{(6)}.}
        \label{tab:pet-pipeline-relation}
    \end{subtable}
\end{table}
